Reducing Tail Latency via Safe and Simple Duplication

Duplication can be a powerful strategy for overcoming stragglers in cloud services, but is often used conservatively because of the risk of overloading the system. We present duplicate-aware scheduling or DAS, which makes duplication safe and easy to use, by leveraging the two well-known primitives of prioritization and purging. To support DAS across diverse layers of a cloud system (e.g., network, storage, etc), we propose the D-Stage abstraction, which decouples the duplication policy from the mechanism, and facilitates working with legacy layers of a system. Using this abstraction, we evaluate the benefits of DAS for two data parallel applications (HDFS, an in-memory workload generator) and a network function (snort-based IDS cluster). Our experiments on the public cloud and Emulab show that DAS is safe to use, and the tail latency improvement holds across a wide range of workloads

==> cloud-eval_tmp.tex <==
\subsection{Cloud Evaluation}
\label{subsec:cloud-eval}
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=0.39\textwidth]{graphs/100vm_cdf.pdf}
  \end{center}
%   \vspace{-0.2in}
  \caption{\sys{} performance on a 100 VM Google Cloud Cluster.}
  \label{fig:cloud_100vm}
    % \vspace{-0.1in}
\end{figure}
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=0.23\textwidth]{graphs/cloud_avg15vm.png}    \includegraphics[width=0.23\textwidth]{graphs/cloud_tail15vm.png}
  \end{center}
%   \vspace{-0.2in}
  \caption{\sys{} performance on a 15 VM Google Cloud Cluster.\asim{Any chance I can have a look at the code?}}
  \label{fig:cloud}
%   \vspace{-0.1in}
\end{figure}

We evaluate \sys{} on the public cloud to quantify its benefits in a real setting, which can potentially have many sources of stragglers. 
We use Google Cloud to conduct our experiments, and compare \sys{} against a single-request system where only a single request is made. 
Our experiments focus on a request-response scenario where a client randomly chooses a server and downloads an object of 10MB. We vary the number of clients and servers for different experiments. The client uses a \texttt{n1-highcpu-16} type VMs while servers use a smaller \texttt{f1-micro} VM. Google provides a big switch abstraction between the VMs -- the server VMs are rate limited to 1Gbps while the client VMs have a limit of 16Gbps\footnote{We observed that instantaneous bandwidth could be higher than these rates, especially after a period of no network activity, suggesting that rate limiting is based on an approach similar to token bucket}. Depending on the offered load in the experiment, the bottleneck could shift between the server and the client network links. 

\paragraph{\sys{} provides substantial gains at both the average and tail request completion times.} 
We use a 100+ VM cluster for our first experiment: there are 100 servers, each running on a separate VM,  and 8 clients running as separate threads on two VMs. The overall load on the system is 10Gbps -- corresponding to 10\% of the aggregate server bandwidth. 
Fig.~\ref{fig:cloud_100vm} shows the CDF of the request completion times for a 30 minute experiment. We observe that \sys{} outperforms a single request system at all levels -- the median request completion times are better by 2x  while the 99th percentile improvement is 3x. 
We also see improvements at lower percentiles -- this is mainly because of \sys{}'s ability to aggregate responses from both the primary and secondary server. The above gains, even for a low load of 10\%, suggest the presence of various stragglers in the real cloud environment. This supports the hypothesis that load imbalance is just one cause for increased tail latency, with various other impairments contributing even at low loads.
%\musa{should request arrival process be mentioned in this section?}

\paragraph{Gains hold across high loads.} To evaluate potential gains of \sys{} at higher loads, we conduct an experiment on a smaller cluster with 1 client and 15 VMs. Fig.~\ref{fig:cloud} shows the responses times as the load increases from 25\% to 75\% of the aggregate server bandwidth. We observe that even at high loads the system remains stable, and more importantly, provides substantial gains (up to 10x for the 99th percentile) over a single request system. We also observed that at very low loads (e.g., up to 25\%), the latency is higher, with the minimum latency for requests achieved at around 50\% load.  We hypothesize that this could be because of specific VM management actions that may kick-in due to inactivity, such as sleep modes, VM preemption, etc. \sys{} is able to deal with such natural stragglers through duplication, reflected by its maximum gains at low loads. 







==> eval-table.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Application} & \textbf{\begin{tabular}[c]{@{}c@{}}Bottleneck\\ Resource\end{tabular}} & \textbf{Settings} & \textbf{Workload} & \textbf{\begin{tabular}[c]{@{}c@{}}Comparison \\ Schemes\end{tabular}} & \textbf{Key Insights} \\ \hline
HDFS & Could be any & Google Public Cloud\cite{google-cloud} & \begin{tabular}[c]{@{}c@{}}Derived from FB Messages Stack \cite{facebookMessages};\\ Request Completion Times(ms)\end{tabular} & Single Copy & \begin{tabular}[c]{@{}c@{}}\sched{} mitigate stragglers in\\  multi-tenant cloud. Minimizes RCTs across all percentiles\end{tabular} \\ \hline

HDFS & Disk & \begin{tabular}[c]{@{}c@{}}Private Cloud \\ (Emulab\cite{emulab})\end{tabular} & \begin{tabular}[c]{@{}c@{}}Same as above\end{tabular} & \begin{tabular}[c]{@{}c@{}}Single Copy, Cloning,\\ Hedged, AppTO\end{tabular} & \begin{tabular}[c]{@{}c@{}}\sched{} is effective and stable across all loads.\\ Purging is key for system stability; Prioritization helps minimize duplication overhead.\end{tabular} \\ \hline

DP-Network & Network & Google Public Cloud \cite{google-cloud} & DCTCP-Search~\cite{dctcp12}, & \begin{tabular}[c]{@{}c@{}}Single Copy,\\  Cloning, Tied\end{tabular} & \begin{tabular}[c]{@{}c@{}}\sched{} naturally deals with flow size heterogeneity, \\ Prioritization provides more gains \\ than purging for short flows.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Evaluation Summary}
\label{table:eval-summary}
\end{table*}









\begin{comment}
\begin{table*}[]
\begin{center}
\footnotesize
    \begin{tabular}{|c|p{1.25cm}|p{1.5cm}|p{1.5cm}|p{5.0cm}|}
    \hline
    Application & Bottleneck Resource & Workload & Comparison Schemes & Key Insights \\ \hline
    HDFS & Disk & Derived from FB HDFS Cluster; Mean time (ms) ~\cite{facebookMessages} & Base, Cloning, Hedged, AppTO, Tied & \sched{} is effective and stable. Naturally deals with disk heterogeneity. Purging is more effective than prioritization, but both are essential at high loads.\\ \hline
    \hkust{} & Network & DCTCP-Search~\cite{dctcp12}, Mean Time ($\mu$s-ms)  & Base, Cloning, Tied  & \sched{} is effective and stable. Naturally deals with flow size heterogeneity. Prioritization provides more gains than purging, but both are essential at high loads\\ \hline
    IDS-Snort & CPU & Synthetic & Base & \sched{} is feasible and can deal with load imbalance\\ \hline
    \end{tabular}
\end{center}
\vspace{-0.1in}
\caption{Evaluation Summary.}
\label{table:eval-summary}
 \vspace{-0.15in}
\end{table*}
\end{comment}


==> figures_text/fig_motivation.tex <==
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=0.40\textwidth]{graphs/SoCC19/Motivation/Motive.pdf}
  \end{center}
   \vspace{-0.2in}
  \caption{A simple experiment to validate the key findings of Table~\ref{table-dup-schemes}. Max-sized bar with black cross indicates that the corresponding scheme becomes unstable.}
  \label{fig:motivation}
%   \vspace{-0.1in}
\end{figure}
